Toward Privacy in Quantum Program Execution On Untrusted Quantum Cloud Computing Machines for Business-sensitive Quantum Needs

Quantum computing is an emerging paradigm that has shown great promise in accelerating large-scale scientific, optimization, and machine-learning workloads. With most quantum computing solutions being offered over the cloud, it has become imperative to protect confidential and proprietary quantum code from being accessed by untrusted and/or adversarial agents. In response to this challenge, we propose SPYCE, which is the first known solution to obfuscate quantum code and output to prevent the leaking of any confidential information over the cloud. SPYCE implements a lightweight, scalable, and effective solution based on the unique principles of quantum computing to achieve this task.

==> sections/background.tex <==
\section{Brief Background Relevant to \sol{}}
\label{sec:background}

In this section, we provide a brief primer on the quantum computing concepts relevant to \sol{}.

\vspace{2mm}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.47]{diagrams/errors.pdf}
    \vspace{1mm}
    \hrule
    \vspace{-3mm}
    \caption{Quantum circuits suffer from various noise-related and operation errors when executed on a quantum computer.}
    \vspace{-3mm}
    \label{fig:errors}
\end{figure}


\noindent\textbf{Qubits and Quantum States.} The fundamental unit of quantum computing is the \textit{qubit}, which is capable of representing a \textit{superposition} (linear combination) of two orthogonal basis states. This is represented as $\ket{\Psi} = \alpha\ket{0} + \beta\ket{1}$, where $\alpha$ and $\beta$ are the complex amplitudes of the constituent basis states. Upon measurement, this superposition collapses such that the probability of measuring the state $\ket{0}$ is $\norm{\alpha}^2$ and $\norm{\beta}^2$ for measuring the $\ket{1}$ state, where $\norm{\alpha}^2 + \norm{\beta}^2 = 1$.

A general system of $n$ entangled qubits is represented as a linear combination (superposition) of $2^n$ basis states: \mbox{$\ket{\psi} = \sum_{k=0}^{k=2^n-1} \alpha_k\ket{k}$}. As with one qubit, when the multi-qubit state is measured, it manifests as a projection to one of the basis states (where now the basis state is a state of $n$ qubits). The probability of measuring state $\ket{k}$ is $\norm{\alpha_k}^2$.

\vspace{2mm}


\noindent\textbf{Quantum Gates and Circuits.} Quantum gates are applied to manipulate the qubit state. The universal basis gate set for IBM's quantum computers (used in this work) consists of the \cx{}, \sx{}, \x{}, and \rz{} gates~\cite{ibmquantum}. \sx{}, \x{}, and \rz{} gates are one-qubit gates. In the Bloch-sphere representation, where a qubit's superposition state is represented on the surface of a sphere, one-qubit gates are categorized by the axis around which the rotation takes place and the angle of rotation. The generalized rotation gate \rz{}$(\theta)$ rotates the qubit state about the z-axis by angle $\theta$. Similarly, the generalized \rx{} gate performs a rotation about the x-axis. While this gate is not a part of the IBM basis, it is used as part of the \sol{} technique (Sec.~\ref{sec:design}) and gets decomposed into the basis gates before hardware execution. Note that \x{}$=$\rx{}$(\pi)$ and \sx{}$=$\rx{}$(\frac{\pi}{2})$.

The \cx{} (controlled \x{}) gate is a two-qubit gate that enables entanglement and applies the \x{} gate to the ``target'' qubit only when the ``control'' qubit is $\ket{1}$. As a note, all of these gates can be represented using unitary matrices. A unitary matrix is a matrix $U$ such that $U^\dagger U = I$, where $U^\dagger$ is the complex conjugate transpose of $U$ and $I$ is the identity matrix.


A quantum program comprises a sequence of one- and multi-qubit gates, as shown in Fig.~\ref{fig:base_circuit}. The sequence is referred to as a \textit{quantum circuit}. A quantum circuit also has a unitary matrix representation, $U$, which can be calculated by taking a Kronecker product of the unitary matrices of all the gates in the circuit in sequential order. At the end of the sequence, some or all of the qubits are measured to get the output. This circuit is prepared and measured multiple times to get a probability distribution over its basis states. \textit{This probability distribution is the output of the quantum program.}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.43]{diagrams/workflow.pdf}
    \vspace{1mm}
    \hrule
    \vspace{-3mm}
    \caption{A quantum algorithm's execution workflow consists of several steps on the user's side as well as the cloud.}
    \vspace{-3mm}
    \label{fig:workflow}
\end{figure}

\vspace{2mm}

\noindent\textbf{Quantum Computing Hardware and Noise.} Currently, there are multiple quantum technologies in different stages of development including superconducting qubits, ion traps, neutral atoms, and photons. While \sol{} is generally applicable to any type of technology, in this paper, we evaluate it on IBM's superconducting-qubit computers as they have the advantage of being relatively easy to fabricate and operate, which has made them a popular choice for quantum computing research~\cite{li2022paulihedral,patel2022quest,balaji2022reliable}. These computers implement a qubit using a Josephson junction, where two superconductors are separated by a thin insulating layer to create a tuneable potential energy barrier for the $\ket{0}$ and $\ket{1}$ states~\cite{patel2020disq}.

A challenge in executing programs on real quantum computers is \textit{hardware noise}, which gives rise to erroneous program outputs. As shown in Fig.~\ref{fig:errors}, errors can occur for different reasons at every stage of the execution of a quantum algorithm. The \textit{state preparation error} refers to the qubit being initialized to the wrong state, and the \textit{measurement error} refers to the error during the measurement procedure. The \textit{gate errors} occur when an operation modifies the qubit incorrectly. These errors are an order of magnitude higher for the \cx{} gates than the \x{} and \sx{}  gates~\cite{patel2020experimental}; \rz{} gates do not have any error as they are implemented virtually using change of reference. \textit{Decoherence} refers to the loss of information due to interaction with the environment occurring over time. 

\vspace{2mm}

\noindent\textbf{Quantum Execution Workflow.} Fig.~\ref{fig:workflow} shows the execution workflow of a quantum computing workload. The user writes the code and compiles the circuit on their end. Then the code is sent to the cloud, where the mapping and routing operations are performed to convert the circuit to a format that can be executed on the qubit connectivity of the selected quantum computer. Note that these steps can also be performed on the user's end, in which case the hardware provider simply runs the circuit. \textit{Where exactly these steps are performed is not of consequence to \sol{}, as \sol{} is applied before these steps are run.} Then, the compiled circuit is run on the hardware, and the output is measured and returned to the user, who processes it for analysis.



==> sections/motivation.tex <==
\section{Related Work and Motivation for \sol{}}
\label{sec:motivation}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.49]{diagrams/related_work.pdf}
    \vspace{1mm}
    \hrule
    \vspace{-3mm}
    \caption{Previous works in quantum privacy have either assumed an untrusted compiler or network model. \textit{\sol{} is the first work to also protect code from an untrusted cloud.}}
    \vspace{-3mm}
    \label{fig:related_work}
\end{figure}

In this section, we review previous work related to achieving privacy in the quantum computing paradigm.

\vspace{2mm}

\noindent\textbf{Quantum Encryption for Communication Networks.} Several previous works have focused on secure quantum network protocols~\cite{xu2023nested,zhang2022instantiation,balaji2022reliable}. As an instance, Balaji et al.~\cite{balaji2022reliable} implement a lattice cryptographic technique to preserve data integrity and resolve the issue of confidentiality over the network using post-quantum encryption with robustness against the Man-In-The-Middle and Sybil attacks. By the same token, Xu et al.~\cite{xu2023nested} propose a system to solve the issue of hiding preambles via random repetition and nested hash coding on multi-domain physical-layer networks. The approach also includes a compression technique based on the concept of quasi-cycle (QC)-moderate-density parity check to encrypt the data in a post-quantum manner. In contrast, Zhang et al.~\cite{zhang2022instantiation} use obfuscation over the network as a form of encryption. The proposed approach utilizes quantum point obfuscation by constructing quantum hash functions, which help enhance the security of the ciphered data. 

\vspace{2mm}

\noindent\textbf{Protection from Third-Party Compiler Software.} Several previous works have focused on protecting quantum code from third-party compilers~\cite{suresh2021short,saki2021split,saki2021survey,phalak2021quantum}. For example, Suresh et al. ~\cite{suresh2021short} attempt to confuse the compiler by adding \cx{} gates, which are removed post-compilation and before hardware execution to get the correct output. Consistent with the above paper, Saki et al.~\cite{saki2021split} propose a split compilation approach where different sections of the code are sent to different compilers so that no one compiler has access to the whole code. The code is stitched back together before hardware execution. On the other hand, Phalak et al.~\cite{phalak2021quantum} propose verification techniques to validate that third-party vendors are indeed dedicating the promised resources to the quantum code. This is done using physically unclonable quantum functions based on superposition and decoherence.


\vspace{2mm}

\noindent\textbf{The Need for \sol{}.} The above works assume that cloud hardware providers are trusted because even if the code is protected from third-party compilers and networks, it still needs to be decrypted before running it on the hardware so that the correct output can be obtained. However, this assumption does not always hold. Even if the cloud is secure, the user may not want to expose their proprietary code to the cloud. However, protecting the code from the cloud is challenging as it requires running the obfuscated code and obtaining the obfuscated output, while also enabling the user to recover the correct output.  Thus, there is a need for a technique to obfuscate the code and output from all non-trusted entities including third-party compilers, the network, and the cloud (Fig.~\ref{fig:related_work}) We design \sol{} to address this challenge.

\vspace{2mm}

\noindent\textbf{Attack Model that \sol{} Tackles.} \sol{} assumes a formidable attacker model, where only the user's local system is trusted. All other components involved in the execution of quantum code including third-party compilers, networks, quantum clouds, and hardware are assumed to be open to attacks. \sol{} protects the user's code from them all.
